Swarm-NG: a CUDA Library for Parallel n-body Integrations with focus on Simulations of Planetary Systems

We present Swarm-NG, a C++ library for the efficient direct integration of many n-body systems using highly-parallel Graphics Processing Unit (GPU), such as NVIDIA's Tesla T10 and M2070 GPUs. While previous studies have demonstrated the benefit of GPUs for n-body simulations with thousands to millions of bodies, Swarm-NG focuses on many few-body systems, e.g., thousands of systems with 3...15 bodies each, as is typical for the study of planetary systems. Swarm-NG parallelizes the simulation, including both the numerical integration of the equations of motion and the evaluation of forces using NVIDIA's "Compute Unified Device Architecture" (CUDA) on the GPU. Swarm-NG includes optimized implementations of 4th order time-symmetrized Hermite integration and mixed variable symplectic integration, as well as several sample codes for other algorithms to illustrate how non-CUDA-savvy users may themselves introduce customized integrators into the Swarm-NG framework. To optimize performance, we analyze the effect of GPU-specific parameters on performance under double precision. Applications of Swarm-NG include studying the late stages of planet formation, testing the stability of planetary systems and evaluating the goodness-of-fit between many planetary system models and observations of extrasolar planet host stars (e.g., radial velocity, astrometry, transit timing). While Swarm-NG focuses on the parallel integration of many planetary systems,the underlying integrators could be applied to a wide variety of problems that require repeatedly integrating a set of ordinary differential equations many times using different initial conditions and/or parameter values.

==> integ_verlet.tex <==
%\subsubsection{Verlet}
%integrator has a small storage requirement than other integrators considered.







==> para_memory.tex <==
\subsection{Data Structures \& Memory Layout}
\label{Sec:MemoryLayout}

Given the considerable computational capabilities of modern GPUs, our program's performance is often limited by memory access.  
Therefore, achieving maximum efficiency requires attention to memory issues such as alignment, coalescing of reads, minimizing bank conflicts, and cache access patterns.  
Considerable effort has been devoted to optimizing memory access patterns in Swarm-NG while maintaining generality and code readability.

Instead of using a data structure containing multiple arrays, Swarm-NG uses arrays of structures.
This results in better spatial locality in the memory, allowing for more efficient memory transfer and caching. 
Furthermore, reducing the number of arrays simplifies memory management and requires fewer registers to store pointers, leaving more registers available for computations.

The data structure for each ensemble of systems is split into two arrays of simple C \ckeyword{struct}s.  
One array holds the information about all bodies in all systems. 
The other array contains information which is stored on a per system basis. 
This is both logically organized and allows for the number of bodies per system to be chosen at run time. 

Since the size of the structures is known at compile time, the compiler can optimize the array indexing at compile time and only a single pointer is required to access all members of the structure. Following C-style data structures where used in the
implementation:

\paragraph{System Structure} 
 A compact C \ckeyword{struct} that holds the current simulation time, an integer containing information about the state of the system, and a provision for an array of additional attributes (e.g., quadrupole moment of central body) that are available for future integrators.  
The number of attributes is set at compile time and easily configurable using \texttt{CMake}.  
The time and attributes are stored in double precision.  
The system data is stored in a one dimensional array of system structures.

\paragraph{Body Structure} 
 A compact C \ckeyword{struct} that contains the position, velocity and mass of the body as well as an array of one or more additional attributes (e.g., radius, composition).  
The number of attributes is set at compile time and easily configurable using \texttt{CMake}.  
All the quantities are stored in double precision.

The body data is stored in a two dimensional array where the inner index is the body number within a system and the outer is determined by the number of the systems within the ensemble.  

However, the accessing scheme is adapted to GPU memory access hardware and thus,
uses some pointer arithmetic in addition to two dimensional indexing.


 


==> verlet_theory.tex <==
The potentially useful integrator with minimal complexity and memory
requirements,  is the time-symmetric, second-order in the time-step ($\Delta t$)
Verlet integrator. Time-reversibility gives it greater stability 
than Euler's method. We implemented Verlet integration with adaptive step-size
according to \cite{Huang1997}.
Ignoring the body indices, the $k$th time step consists of
%
\begin{itemize}
\item First half of a drift step: \\
${\textbf x}_{k+\frac{1}{2}} \colon= {\textbf x}_k + \frac{1}{2}{\textbf v}_k\Delta t_{k-1}$
\item Step-size adaptation: \\
	$\Delta t_k \colon= [(g({\textbf x}_{k+\frac{1}{2}})\Delta\tau_{\mathrm{max}})^{-1}-(\Delta t_{k-1})^{-1}]^{-1}$
\item Kick step:  \\
	${\textbf v}_{k+1} \colon= {\textbf v}_k + \frac{1}{2} {\textbf a}_k({\textbf x}_{k+\frac{1}{2}}) (\Delta t_{k-1} + \Delta t_{k})$
\item Second half of a drift step: \\
	${\textbf x}_{k+1} \colon= {\textbf x}_{k+\frac{1}{2}} +\frac{1}{2} {\textbf v}_{k+1}\Delta t_k$
\end{itemize}
%
The constant $\Delta\tau_{\mathrm{max}}$ is the maximum time-step.
Based on physical intuition from the 2-body problem, 
%
\be
g({\textbf x}) := \left[\left(1+\tau_o^2 \left(\sum_{j\neq i} \frac{G\left(m_i+m_j\right)}{|{\textbf x}_j-{\textbf x}_i|^3}\right)\right)^{\frac{1}{2}}\right]^{-1},
\ee
%
where $\tau_o$ sets the timescale below which the time-step transitions from a constant ($\tau_{\mathrm{max}}$) to decreasing with the local orbital timescale.  
This results in a time-step that scales with the minimum local orbital
time scale of any pair of bodies, subject to a maximum time-step of $\tau$.  
Verlet was the first algorithm implemented in Swarm-NG.
It is now deprecated in favor of the
following more sophisticated integrators.

